Decoding FL Defenses: Systemization, Pitfalls, and Remedies

While the community has designed various defenses to counter the threat of poisoning attacks in Federated Learning (FL), there are no guidelines for evaluating these defenses. These defenses are prone to subtle pitfalls in their experimental setups that lead to a false sense of security, rendering them unsuitable for practical deployment. In this paper, we systematically understand, identify, and provide a better approach to address these challenges. First, we design a comprehensive systemization of FL defenses along three dimensions: i) how client updates are processed, ii) what the server knows, and iii) at what stage the defense is applied. Next, we thoroughly survey 50 top-tier defense papers and identify the commonly used components in their evaluation setups. Based on this survey, we uncover six distinct pitfalls and study their prevalence. For example, we discover that around 30% of these works solely use the intrinsically robust MNIST dataset, and 40% employ simplistic attacks, which may inadvertently portray their defense as robust. Using three representative defenses as case studies, we perform a critical reevaluation to study the impact of the identified pitfalls and show how they lead to incorrect conclusions about robustness. We provide actionable recommendations to help researchers overcome each pitfall.

==> cover_letter.tex <==
% This work started off as a paper at the DLSP workshop at IEEE S\&P 2023. There we initiated the identification of FL pitfalls in FL defenses and used FedRecover as a case study to assess the impact of four pitfalls.
% The DLSP paper was the first step in the direction of this paper, where we identify two more pitfalls, and use another SOTA defense FLDetector as a case study. Here, before diving into the pitfalls and their prevention, we found it important to first classify defenses according to their working mechanisms so that it becomes easier to understand the choice of our defense mechanism selection. It also makes a natural transition from systemization to pitfalls because in systemization we thoroughly explain how different defenses work and how they are different from each other. We then proceed to pitfalls and their impact analysis in the paper. In this paper, we not only perform a lot more experiments but also a much more extensive analysis of pitfalls, their impact, and our recommendations. We also include a large-scale evaluation using the very large StackOverflow dataset, something which the workshop paper lacked. Using StackOverflow also helped us expand our study into the language domain, as the workshop paper only had image datasets and models. The difference in scope of evaluation and analysis is clearly evident by the number of figures in both papers. The workshop paper has 5 figures, while this paper has 15. The overlap that exists between the two papers is because this paper builds upon the previous one and we had to use the first four pitfalls in our current study as well. Therefore, we performed more experiments and analysis with the first four pitfalls, while also including two new pitfalls.



Dear Editor-in-chief,

We are submitting our manuscript for consideration for publication in ACM Transactions on Privacy and Security (TOPS). This work builds upon our earlier workshop paper presented at the IEEE DLSP Workshop at IEEE S\&P 2023. While the workshop paper provided an initial exploration of pitfalls in Federated Learning (FL) defenses using FedRecover as a case study, the current journal submission significantly expands both the scope and depth of our investigation.

In our workshop paper, we identified and analyzed the impact of four key pitfalls. The current paper not only revisits these pitfalls with additional experiments and in-depth analysis but also identifies two new pitfalls, thereby extending the conceptual framework. Furthermore, we introduce a novel systemization for FL defenses based on their working mechanisms, providing a systematic perspective that aids in understanding the rationale behind our choice of defense mechanisms. This systemization forms a natural progression into our expanded study of pitfalls and their prevention.

A significant enhancement in this work is the scale and diversity of evaluation. Unlike the workshop paper, which focused exclusively on image datasets and models, the present study includes a large-scale evaluation using the StackOverflow dataset. This addition allows us to extend our analysis to the language domain, demonstrating the broader applicability of our findings. The difference in scope is also reflected in the volume of results and visualizations: the workshop paper included 5 figures, whereas the current submission contains 15 figures to comprehensively present our findings.

The overlap between the two papers arises naturally from the progression of the research, as we revisit the initial four pitfalls in light of new experiments and integrate them into the broader framework developed in this submission. This overlap is limited to foundational aspects that were essential to build upon and is complemented by the substantial new contributions in this paper.

We believe that the manuscript represents a significant advancement over the workshop paper and will be of interest to the readership of ACM TOPS. We have ensured that all necessary citations to the prior work are included.

Thank you for considering our submission. We look forward to the possibility of contributing to ACM TOPS.

Sincerely,
Authors

==> method.tex <==
\section{Methodology}\label{sec:method}

\begin{figure*}
\centering
\includegraphics[scale=.4]{figures/defenses_survey.pdf}
% \vspace*{-0.8cm}
\caption{Frequency of choices of the six key components (Dataset, distribution of clients' data, FL algorithm, FL type, attacks, and evaluation) of robustness evaluation setup. \S~\ref{sec:impact} discusses the impacts of choices on the robustness of FL poisoning defenses.}
\label{fig:defense_survey}
% \vspace*{-.5cm}
\end{figure*}

\textcolor{red}{describe why this section was needed. basically you are providing the descriptions for some of the components being used later so the reader can know them early on. For example, you will describe FedSGD/FedAvg, cross-silo/cross-device here.\\
Here you are explaining the components of FL workflow. In the pitfalls section you are explaining the pitfalls in the workflow. There is a big difference. Then later on you are explaining the impact. These three need to be separately explained. Make sure you explain this properly for the reader!\\
Also decide the order of components/pitfalls 3 and 4}
\begin{itemize}
    \item Papers selection
    \item FL components selection
    \item Pitfall identification
    \item Re-evaluation methodology
    \item Also mention that you use many tasks and modalities, i.e., image classification, next-word prediction, and human activity recognition using multimodal sensor data.
\end{itemize}

% \noindent\textbf{The Federated Learning workflow:}
\subsection{The Federated Learning workflow:}\label{method:workflow}
Federated Learning comes in many variants, but we divide a typical FL defense evaluation workflow into six distinct components. Below, we briefly explain the components in the order they typically appear in the workflow(~\ref{fig:fl_flowchart}):
\begin{itemize}
    \item Dataset: The first step in any learning-based system, including FL, is to select or collect a dataset for evaluation. We report the prevalent datasets in ~\S\ref{pitfalls:1}, and through a thorough evaluation, assess the impact of the different choices of these datasets in ~\S\ref{impact:datasets}.
    \item Data Distribution: If a dataset such as MNIST or FashionMNIST is used for evaluation, it must first be distributed among the clients participating in the FL training using some distribution technique such as Dirichlet Distribution~\ref{}. On the other hand, some datasets are specifically designed for FL evaluations, e.g., FEMNIST(~\cite{caldas2018leaf}). In ~\ref{pitfalls:2}, we report the prevalence of such techniques, and in ~\S\ref{impact:distribution}, we show the difference between these distributions and their impact on FL robustness.
    \item FL Type: Once data has been distributed among clients, we have to decide the policy for client selection in every round of FL, which we refer to as the \emph{FL Type}.
    The FL type for practical deployments can be either \textbf{cross-device} or \textbf{cross-silo}~\cite{kairouz2019advances}. In \emph{cross-device FL}, the total number of clients, $N$, is very large (from a few thousand to billions), and only a tiny fraction of them is chosen in each FL training round, i.e., $n\ll N$. Clients are resource-constrained devices such as mobile phones, smartwatches, IoT devices, etc. While, in \emph{cross-silo FL}, $N$ is moderate (up to 100), and all clients are selected in each round, i.e., $n=N$, where clients are large corporations, e.g., banks, hospitals, etc. \textcolor{red}{prevalence and implications}
    \item FL Algorithm: Another important step in the FL workflow is to decide how local and global updates will be computed. Based on how these updates are computed, we can classify FL Algorithms into two types: FedSGD and FedAvg~\cite{mcmahan2017communication}, whose update computation we have described in~\S\ref{background:FL}. We report the prevalence of these FL algorithms in~\S\ref{pitfalls:3} and the impact of FedAvg over FedSGD in~\S\ref{impact:algorithm}.
    \item Attack: Once the above four components have been selected, the attack needs to be chosen. There are different kinds of attacks designed for FL, which we thoroughly explain in~\S\ref{background:attacks}. We find in our study that many naive attacks are commonly used~\S\ref{pitfalls:5}, and stronger adaptive attacks lead to different conclusions on the robustness of FL defenses~\S\ref{impact:attacks}.
    \item Evaluation Metrics: The final step in the FL evaluation workflow is to choose the metrics to be computed and reported. Since there are multiple parties collaborating in FL, in addition to a server, the metrics can be different for each of them. We show in~\S\ref{pitfalls:6} that most of our surveyed works report the server's metrics, and in~\S\ref{impact:evaluation}, we compare the global metrics with local ones and find drastic differences between the two.
\end{itemize}

% \noindent\textbf{Papers selection:}
\subsection{Papers Selection:}\label{method:selection}
We select 50 FL defense papers from top-tier security venues: Usenix Security, IEEE S\&P, ACM CCS, and NDSS, and identify the six components(~\S\ref{method:workflow}) of FL workflow for each of them. We list the surveyed papers in Table~\ref{tab:defenses}, and mention the choices for each of the six components. We then plot the frequency of these choices to get a better understanding of the prevalent choices in Figure~\ref{fig:defense_survey}.

\subsection{Re-evaluation Methodology:}\label{method:reevaluation}
\textcolor{red}{Write here how you will perform the re-evaluation. In the background section you justified the choice of attacks and defenses used. Here explain how you will perform the reevaluation. i.e., re-implementation, baselines, experimental setup. All of that goes here. Also mention limitations of your reevaluation here. Such as not being able to perform all settings on all defenses. Some due to practical limitations. Some due to space limitations.}



==> review.tex <==
Review #888A
===========================================================================

Paper summary
-------------
This paper tries to reevaluate existing defenses against attacks to federated learning. In particular, the paper tries to identify weaknesses in the evaluation of existing defenses.

Strengths / Reasons to accept
-----------------------------
1. The work surveys many existing defenses against untargeted model poisoning attacks to FL.

2. In general, the paper is not hard to follow.

Weaknesses / Reasons to reject
------------------------------
1. This paper is closely related to [43]. In particular, many figures and results from [43] are used as the results/findings of this paper, but [43] is not cited for those results/findings. Given [43] is formally published, the authors may consider citing [43] when the results/findings from [43] are used.

Answer: Cite major results from [43], and try to use different results wherever possible.

2. In pitfall-1, it is recommended that more complex datasets could be used in evaluation. This is very straightforward. Additionally, it is recommended that datasets like FEMNIST and CIFAR10 can be used. Those datasets are also toy datasets as they cannot represent real-world scenarios of FL.

Answer: Re-phrase your recommendation to use FEMNIST and CIFAR10. CIFAR10 is a toy dataset but it should be distributed according to techniques that mimic real world distributions, e.g., Dirichlet Distribution. FEMNIST is a dataset designed for FL specifically so here the reviewers comment is not justified.

3. It is assumed that 20\% of clients are malicious, which is very high. In other words, this setting may not be realistic in the real world for both cross-device and cross-silo FL. As pointed out by the authors, the evaluation of both attacks and defenses heavily relies on the settings. Thus, a systematic evaluation for a different fraction of malicious clients is needed. Same for many other hyperparameters.

Answer: We use 20\% malicious clients to match the settings in the previous papers to compare our results with them.
TODO: Make a graph that shows the impact of varying percentages of malicious clients.

4. Only three defenses are evaluated in Section 5, making the conclusions less convincing. More defenses could be evaluated since the major contribution of this paper is evaluation.

Answer: bruh. read the systemization section.

5. It is unsurprising that attacks are more effective while defenses are less effective for higher data heterogeneity. Additionally, there is always a tradeoff between security and utility. Therefore, it is unclear whether it is possible to develop perfect defenses under high data heterogeneity.

Answer: That is the point we are trying to make. Many defenses are evaluated only under low-heterogeneity/IID settings and they fail under non-iid settings. IID data distribution is extremely non-practical, hence we term this approach a pitfall.


6. The evaluation is limited to untargeted model poisoning attacks, leaving other attacks such as backdoor attacks unexplored.

Answer: We used untargeted model poisoning attacks because they are the strongest.
TODO: Use some targeted attack for your evaluation as well(If time).

In summary, it would be more convincing if the evaluation is conducted on a FL system that is deployed in the real world. Otherwise, it is less convincing which settings are more realistic. Additionally, the evaluation is not very systematic, which may lead to biased conclusions. Finally, results/findings from [43] should be properly cited as [43] is formally published.

Does the paper raise ethical concerns?
--------------------------------------
1. No

Reviewer expertise in this domain
---------------------------------
3. Knowledgeable (I don't necessarily work in this topic domain, but I work
 on related topics or I am cognizant of the work in this domain in recent
 years)

Reviewer confidence
-------------------
3. Quite confident

Overall merit
-------------
1. Reject


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #888B
===========================================================================

Paper summary
-------------
This paper is a systematization study of the plethora of defenses that have been proposed against poisoning attacks in federated learning. In particular, the focus is on the pitfalls of defenses against untargeted model poisoning attacks, which modify model parameters in order to lower the test accuracy of the global model. The paper uses 3 defenses (Trimmed Mean, FL Detector and FL Recover) to illustrate salient pitfalls in their evaluation. The experimental evaluation highlights how defense strengths may have been overestimated by not considering a wide range of datasets, client-wise distributions and adaptive attacks. The paper provides recommendations for future evaluation of defenses.

Strengths / Reasons to accept
-----------------------------
- The paper represents a good effort towards unifying the themes that guide the creation of defenses against model poisoning attacks, particularly untargeted ones. The identified pitfalls are useful ones for defenses proposed in the future to be aware of, and the overview provided in Table 1 effectively captures the scope of existing defenses in terms of their actions and knowledge.
- The 3 defenses chosen to illustrate the pitfalls are reasonable, covering different defenses philosophies around direct parameter modification, detection of malicious updates and post-facto restoration of models.
- The proposed adaptive attack on FL Detector is a good attempt at demonstrating how adaptive adversaries can bypass defenses that are not provably robust under practical conditions.

Weaknesses / Reasons to reject
------------------------------
- I think the paper misses a trick by completely ignoring targeted attacks. These present a different challenge for defenses as they are much stealthier, but weaker. In some cases, they may be worse since models could be deployed with ostensibly high performance on the test/validation data but have triggered or triggered backdoors embedded that cause misclassification. It would be very interesting to see if the same pitfalls exist, and if defenses proposed against untargeted attacks are able to tackle the stealthier mode in which targeted attacks operate.

Answer: We used untargeted model poisoning attacks because they are the strongest.
TODO: Use some targeted attack for your evaluation as well(If time).


------------------------------------------------------------------------------------------------------------------------------------------------------------
- While the considered fraction of malicious clients (20\%) is good from the perspective of considering strong attackers, the paper needs to ablate over different malicious client percentages to understand how realistic proposed attacks are, and if stronger attacks are also something the community needs to focus on. While Section 5.4 does consider how FL systems can be intrinsically robust in the cross-device setting, it does not consider powerful attacks that have been proposed in the targeted setting such as Neurotoxin (Zhang et al., ICML 2022), which need far smaller fractions of malicious clients.

Answer: again, we did that to match our results to previous works. how can we compare otherwise?
TODO: perform the percentage of malicious clients ablation.
---------------------------------------------------------------------------DONE-----------------------------------------------------------------------------


- The paper does not consider heterogenity-aware aggregation mechanisms such as agnostic federated learning (Mohri et al., ICML 2019), which account for a diversity of distributions across clients. There are other popular averaging algorithms such as Matched Averaging as well (Wang et al., ICLR 2020) which operate in a layer-wise fashion. For a systemization paper, there needs to be more focus on the aggregation mechanisms used as these will have a large impact on the success of proposed attacks.

TODO: See if you have time to include one of these aggregation mechanisms.

- I found the conclusions in 5.1 and 5.2 to be largely identical, since both revolve around the concern of sufficient heterogenity in benchmark datasets. Also, Section 5.5.2. relies too much on prior knowledge of FLDetector. The paper would benefit from a better description of these defenses that then brings out the novelty of the adaptive attack.

TODO: Re-phrase your findings in these sections.

- One of the defenses considered for a detailed analysis should have been a provable one like CRFL, to see if the assumptions under which they are provably robust hold in practice.

Constructive comments for author
--------------------------------
See Strengths and Weaknesses

Questions for authors’ response
-------------------------------

------------------------------------------------------------------------------------------------------------------------------------------------------------
- Why does the accuracy increase monotonically with the client number in Figure 12?
Answer: It does not monotonically increase. It is sorted in ascending order and then plotted.
---------------------------------------------------------------------(DONE)---------------------------------------------------------------------------------

------------------------------------------------------------------------------------------------------------------------------------------------------------
- Isn’t Pitfall 4 really more of an attack pitfall, since supposedly stronger attacks should consider how effective they are in cross-device settings?
TODO: Re-phrase to clarify that it isn't an attack pitfall.
---------------------------------------------------------------------(DONE)---------------------------------------------------------------------------------

Does the paper raise ethical concerns?
--------------------------------------
1. No

Concerns to be addressed during the revision/shepherding
--------------------------------------------------------
See Strengths and Weaknesses, but overall I think the paper needs more work to come to crisper and more interesting observations about the interaction between attacks and defenses in FL.

Reviewer expertise in this domain
---------------------------------
4. Expert (I've worked on this topic domain or a closely related topic
 domain)

Reviewer confidence
-------------------
4. Confident

Overall merit
-------------
2. Weak reject

==> revision.tex <==
\section{\textit{\textbf{REVIEWER 1}
}}

1. In Section 2.2.3, it is said that "three representative defense techniques" are chosen since "they are distinct in their nature." However, it is not explained what the "nature" of these defense techniques is. More specifically, there is a lack of overview of existing defense works, thus it is difficult to judge whether the three chosen defense techniques are representative or not. As far as I am concerned, both Trimmed Mean and FLDetector try to detect and remove malicious participants (Don't they belong to the same type of defense?) and FedRecover tries to recover the correct model without detection. Additionally, TrMean is an early work (2018), thus its limitations may not apply to more recent defense works.

\textbf{\textit{Response:}}
Trimmed Mean removes malicious components of updates dimension-wise and the training continues til completion i.e., until the end of specified global rounds. FLDetector, on the other hand, detects malicious clients, removes them from the client pool entirely, and then restarts the training process.
Trimmed Mean is an early work but it has been used in recent works (cite FedRecover, Back to the Drawing Board,  FLDetector), hence we include it in our study as a representative 'filtering' defense.

2. In Pitfall-2, the highlighted statement "high heterogeneity can make us believe that a system is robust when it is not" is confusing. It is shown by experiments in the paper that high heterogeneity makes a system less robust. I suggest clarifying this statement.

\textbf{\textit{Response:}}
Changed statement to "low heterogeneity can make us believe that a system is robust when it is not".

3. In Pitfall-3, the title is "Incorrect Baselines." I find it inappropriate since the authors did not refer to baselines (i.e., other defense works that a proposed defense work is to be compared with), but rather the federated learning algorithms.

\textbf{\textit{Response:}}

4. In Pitfall-4, the statement "Considering only hypothetical scenarios, while ignoring practical limitations..." is too vague. It can refer to almost anything. In this part, the authors actually want to explain that existing defenses usually assume a cross-silo rather than a cross-device FL setting. This is not "hypothetical scenarios" but only "limited scenarios." Additionally, it has already been found that poisoning attacks are less effective in a cross-device FL setting than in a cross-silo FL setting, thus evaluating defenses against stronger attacks (i.e., the cross-silo setting) may not be faulty, in my humble opinion.

\textbf{\textit{Response:}}
Consider changing this to:
Pitfall-4: Limited FL Setting. Considering limited settings, such as using only small-scale settings for evaluations, may not lead to conclusions that apply to large-scale settings as well.
In its explanation, write that with scaling up the system, the threat model changes (cite back to the drawing board). And since the threat model changes, e.g., it becomes more stricter about the percentage of malicious clients in cross-device, the attacks naturally become less effective and defenses naturally become more effective.

5. In Section 4.2 (Stat-1), the statement "We note that Dir produces client datasets ... very similar to those of the real-world datasets in Leaf repository" is unsupported. The authors need to give a reference to the Leaf repository, or better still, show the distribution of real-world datasets in the Leaf repository.

\textbf{\textit{Response:}}
Include the FEMNIST data distribution figure from the leaf website.

6. In Section 5.1, it is concluded that on a large scale, poisoning attacks are ineffective and simple AGRs are unaffected. This conclusion has already been reached in existing works [1].
[1] Shejwalkar, Virat, et al. "Back to the drawing board: A critical evaluation of poisoning attacks on production federated learning." 2022 IEEE Symposium on Security and Privacy (SP). IEEE, 2022.

\textbf{\textit{Response:}}
Our experiments differ from [1] in a way that we evaluate using an actual real-world dataset that is naturally distributed with 130 million training samples and 300,000 users.

7. In Section 5.2, I am confused by the Recommendation "we propose to balance data..." It seems that a lot has been argued for an imbalanced dataset setting. Did the authors mean that we should balance the data only for the multimodal sensing datasets or imbalanced datasets? I also find that the two questions raised in this section "(1) How does imbalance among classes in train and test data affect the robustness of a system? and (2) How do choice of evaluation metrics impact our assessment of the robustness of a system" unanswered.

\textbf{\textit{Response:}}

8. There are many typos and non-standard expressions in the paper, including but not limited to:

- I suggest referring to [74] by another name rather than "NDSS attack".
- "L-BFGS" or "LBFGS", please be consistent.
- replace "iid" with "i.i.d."
- replace "Fcj" with "FCJ"
- What is hvp in page 9?
- What is %m in Table 2?
- The title of Section 5.2 "Mumltimodal" should be "Multimodal"

\textbf{\textit{Response:}}
-
-done
-done
-done
-
-
-done


\section{\textbf{\textit{REVIEWER 2}}}

(i) Premise of paper: When I set out to read the paper, I originally thought that this would be an SoK-style one; however, after reading, it seemed the first half was more of an SoK, and second half was about the authors proposing a new adaptive attack. I found the storyline of the paper to be confusing and could not easily follow the logical coherence between each section. I would suggest the authors to either stick to an SoK paper and provide more details about the analysis of the 50 top-tier papers they selected.

\textbf{\textit{Response:}}
Change writing in a way that it appears as an SoK/survey/analysis paper. But present the adaptive attack as a byproduct of your re-evaluation. Show that you needed the adaptive attack to prove the point about choice of attacks, and that it is not the standalone contribution of your paper.

(ii) Paper title: currently, the title is too broad/generic and I would recommend the authors to use a title that is more representative of the work they present in the paper. “En Route Robust Federated Learning” does not make any sense and “A Critical Analysis of Experimental Practices in Security Evaluation” is also misleading as the authors only focus on defense papers against poisoning attacks.

\textbf{\textit{Response:}}
The title should mention something about the experimental setups of defenses, and that we are performing a re-evaluation of existing defenses with different settings.

(iii) Introduction: on page 2, column 1, the authors do mention the existing works that identify pitfalls in machine-learning based security; however I miss a justification for why the authors think that the pitfalls that they identified and proposed in this work are different from the ones that have been already put forward by previous work. A justification on what makes FL unique would help the reader to better understand why such a study is required. At the moment, my impression is that there is almost a 100\% overlap between the pitfalls mentioned in this paper and the ones from the literature.

(iv) Set of 50 top-tier papers: There is no clarification as to how these papers were selected. As the authors pointed out, there exists a large body of work on defense papers for FL; however, I miss an explanation as to why these specific papers were selected. An explanation on the selection method and criteria would be much appreciated.

\textbf{\textit{Response:}}
Write a section explaining the paper selection methodology.

(v) Section 2.2: The sub-heading could again be a bit more descriptive. You wrote “Poisoning attacks against FL”, but you also present three defenses in section 2.2.3. 

Regarding section 2.2.1: I do not follow the justification for the percentage of malicious clients you considered in your threat model. In the footnote, you wrote “Most defense works assume very high percentages of malicious clients to demonstrate that their defenses work even in highly adversarial settings. Hence, although unreasonable in practical FL settings [73], we follow prior defense works and use 20\% malicious clients.” If the assumption made by prior work is unreasonable in practical FL, why did you then follow prior work? Or did you mean to phrase this assumption differently and intended to stay consistent with assumptions made by prior works?

Section 2.2.2: please define what is NDSS attack.

\textbf{\textit{Response:}}
Change the footnote to add we choose 20\% malicious clients to stay consistent with the assumptions made by prior works.

Change the NDSS attack to Dyn-Opt(Dynamic Optimization)


(vi) Section 3: This whole section seems disconnected form the rest of the paper. I did not understand why would the authors state the pitfalls, explain their prevalence and implications, and immediately present recommendations. The observations made in the Prevalence and Implications seem unfounded and I could not follow how the authors came to the conclusions they presented. Moreover, I miss an explanation on how the pitfalls were identified (this further strengthens my point regarding the overlap with existing works that also studied pitfalls). There was also no connection with the content of section 3 to what was presented in section 2.2. How did the authors, after considering 2 attacks and 3 defenses, already came up with the 6 pitfalls they presented?

\textbf{\textit{Response:}}
Convert the paper to SoK style. And explain clearly in the beginning why you are structuring the paper in a particular way so that the reader knows clearly in the beginning what the purpose of this structure is.

(vii) Section 4: This section gets even more confusing. After having already provided recommendations for the pitfalls, the authors now evaluate the impact of the proposed pitfalls on FL security. What is the connection between the recommendations in section 3 and the evaluation in section 4?

\

(viii) Section 5: The section heading says “Analysis of Hidden Pitfalls in FL Security” - how were the hidden pitfalls identified or discovered? Is there any connection between the six pitfalls and hidden pitfalls in section 5? What role did the set of 50 top-tier paper play in identifying the hidden pitfalls?

\textbf{\textit{Response:}}
Explain that section 5 is different from section 3 and 4. The 6 pitfalls mentioned are related to different experimental settings that are already known and used in literature. For example, the FEMNIST dataset has still been used in the top-tier 50 papers. But there is no paper in those 50 that discusses multimodal sensor data. Or a large-scale NLP task. Therefore we set aside a separate category.
Think of a reason for why they imbalanced data case is something different from the 6 pitfalls and why you wrote it separately.

(ix) Discussion: Given that this paper evaluated a large body of defense papers for FL systems, I would have expected a section discussing the findings and impact on future research challenges. It could be that since the authors got side-tracked into implementing a new adaptive attack, took away the primary focus of what this paper should have been about.

\textbf{\textit{Response:}}
Make changes to the writing so that the paper does not seem like it is centered around the adaptive attack. Explain clearly that the adaptive attack is the byproduct of your re-evaluation methodology, and it was necessary to design an adaptive attack to show that FLDetector does not perform up to the mark in the presence of adaptive attacks.

==> sketch.tex <==
Revision major
Think of a better representation of "sec 5: Analysis of Hidden Pitfalls in FL Security"


---------
Pitfalls identification  (figure would be great)
Datasets -- all
Data distribution --- all
FL type -- Cross silo all, but only trimmean cross device
FL algorithm -- all
Attacks -- all
Evaluation -- Trimmean, Fedrecover
----------
defense classes (figure would be great):
-Filtering -- Trimmean
-Detection -- FLdetector
-Recovering -- Fedrecover

Section reference ~\S\ref{defenses:classification:method}.
